Smart Street Lights and Mobile Citizen Apps for Resilient Communication in a Digital City

Currently, nearly four billion people live in urban areas. Since this trend is increasing, natural disasters or terrorist attacks in such areas affect an increasing number of people. While information and communication technology is crucial for the operation of urban infrastructures and the well-being of its inhabitants, current technology is quite vulnerable to disruptions of various kinds. In future smart cities, a more resilient urban infrastructure is imperative to handle the increasing number of hazardous situations. We present a novel resilient communication approach based on smart street lights as part of the public infrastructure. It supports people in their everyday life and adapts its functionality to the challenges of emergency situations. Our approach relies on various environmental sensors and in-situ processing for automatic situation assessment, and a range of communication mechanisms (e.g., public WiFi hotspot functionality and mesh networking) for maintaining a communication network. Furthermore, resilience is not only achieved based on infrastructure deployed by a digital city's municipality, but also based on integrating citizens through software that runs on their mobile devices (e.g., smartphones and tablets). Web-based zero-installation and platform-agnostic apps can switch to device-to-device communication to continue benefiting people even during a disaster situation. Our approach, featuring a covert channel for professional responders and the zero-installation app, is evaluated through a prototype implementation based on a commercially available street light.

==> eval_tabs/computestick.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of Concept Detection on Pi vs. Neural Compute Stick}
\label{sec:eval:stick:power}
\begin{tabular}{@{}rllrllrllr@{}}
\toprule\multicolumn{1}{r|}{} & \multicolumn{3}{c}{\textbf{Idle} - Power in mW} & \multicolumn{3}{c}{\textbf{Starting} - Power in mW} & \multicolumn{3}{c}{\textbf{Analysis} - Power in mW}\\ 
\multicolumn{1}{r|}{} & Mean & Max & Time & Mean & Max & Time & Mean & Max & Time per Image\\ 
\midrule 
\multicolumn{1}{r|}{Pi 3b, 1K, CPU} & 1107 & 1845 & 59.29 sec. & 2626 & 2895 & 19.66 sec. & 2723 & 3537 & 13.27 sec. \\
\multicolumn{1}{r|}{Pi 3b, 1K, Movidius} & 1955 & 2095 & 59.76 sec. & 2372 & 2884 & 3.92 sec. & 2760 & 3388 & 0.61 sec. \\
\multicolumn{1}{r|}{Pi 3b, 6K, CPU} & 1107 & 1845 & 59.29 sec. & 2659 & 3203 & 75.03 sec. & 2871 & 3537 & 5.46 sec. \\
\multicolumn{1}{r|}{Pi 3b, 6K, Movidius} & 1955 & 2095 & 59.76 sec. & 2507 & 2879 & 12.64 sec. & 3313 & 3667 & 0.82 sec. \\\bottomrule
\end{tabular}
\end{table*}


==> eval_tabs/cost_modem.tex <==
\begin{table}[H]
\centering
\caption{Cost of BLE LoRa Modem}
\label{sec:eval:cost:modem}
%\begin{tabularx}{\columnwidth}{@{}lcl@{}}
\begin{tabular}{@{}lrl@{}}
\toprule
\textbf{Part}          & \multicolumn{1}{l}{\textbf{Estimate Price}} & \textbf{Comment} \\ \midrule
TTGO LoRa SX1276 ESP32 & 9 €                                         & incl. antenna    \\
LiPo Battery 750mAh    & 3 €                                         &                  \\
3D printed case        & 2 €                                         &                  \\ \midrule
\textbf{Total Price}   & 14 €                                        &                  \\ \bottomrule
%\end{tabularx}
\end{tabular}
\end{table}

==> eval_tabs/cost_msp.tex <==
\begin{table}[h]
\centering
\caption{Example configuration for a MSP}
\label{sec:eval:cost:msp}
%\begin{tabularx}{\columnwidth}{@{}lcl@{}}
\begin{tabular}{@{}lrl@{}}
\toprule
\textbf{Part}                   & \multicolumn{1}{l}{\textbf{Estimate Price}} & \textbf{Comment} \\ \midrule
TTGO LoRa SX1276 ESP32          & 9 €                                         & incl. antenna    \\
LiPo Battery 1500mAh            & 3 €                                         &                  \\
3D printed case                 & 4 €                                         &                  \\
Ublox NEO GPS                   & 12 €                                        & incl. antenna    \\
SD-Card Breakout                & 2 €                                         &                  \\
32 GB SD Card                   & 13 €                                        &                  \\
Real Time Clock 				& 1 €                                         &                  \\
Temperature  \& Humidity Sensor & 1 €                                         &                  \\
Gyro Sensor                     & 1 €                                         &                  \\ \midrule
\textbf{Total Price}            & 46 €                                        &                  \\ \bottomrule
%\end{tabularx}
\end{tabular}
\end{table}


==> eval_tabs/cost_ssp.tex <==
\begin{table}[H]
\centering
\caption{Example configuration for a SSP (w/o power supply)}
\label{sec:eval:cost:ssp}
%\begin{tabularx}{\columnwidth}{@{}lcl@{}}
\begin{tabular}{@{}lrl@{}}
\toprule
\textbf{Part}                   & \multicolumn{1}{l}{\textbf{Estimate Price}} & \textbf{Comment}           \\ \midrule
Raspberry Pi 3                  & 32 €                                        &                            \\
TTGO LoRa SX1276 ESP32          & 9 €                                         & incl. antenna              \\
3D printed case                 & 10 €                                        &                            \\
Ublox NEO GPS                   & 12 €                                        & incl. antenna              \\
32 GB SD Card                   & 13 €                                        &                            \\
Real Time Clock 				& 1 €                                         &                  \\
Temperature  \& Humidity Sensor & 1 €                                         &                            \\
Pi Camera                       & 20 €                                        & night vision opt. \\
\textit{Movidius NCS}           & \textit{66 €}                               & \textit{optionally}        \\
Thermal Imaging                 & 32 €                                        &                            \\
Rain Sensor                     & 1 €                                         &                            \\
Soil Moisture                   & 3 €                                         &                            \\
PIR Motion Detector             & 1 €                                         &                            \\ \midrule
\textbf{Total Price}            & 135 €\textit{ / 201 €}                      &                            \\ \bottomrule
%\end{tabularx}
\end{tabular}
\end{table}

==> eval_tabs/platforms.tex <==
\begin{table*}[ht!]
\centering
\caption{Overview of SBC and MCU Platforms}
\label{sec:eval:plat:platforms}
\begin{tabular}{@{}rlllrrrr@{}}
\toprule\multicolumn{1}{r|}{} & \textbf{Processor} & \textbf{RAM} & \textbf{Network} & \multicolumn{2}{c}{\textbf{Idle} - Power in mW} & \multicolumn{2}{c}{\textbf{Load} - Power in mW}\\ 
\multicolumn{1}{r|}{} &  &  &  & Mean & Max & Mean & Max\\ 
\midrule 
\multicolumn{1}{r|}{Pi 1 Model B+} & 1x 700 MHz & 512 MB & 100 Mbit Eth. & 931 & 1288 & 1043 & 1418 \\
\multicolumn{1}{r|}{Pi 3 Model B} & 4x 1200 MHz & 1024 MB & 100 Mbit Eth., WiFi, \faBluetooth~4.1 & 1107 & 1845 & 2224 & 3285 \\
\multicolumn{1}{r|}{Pi Zero W} & 1x 1000 MHz & 512 MB & WiFi, \faBluetooth~4.1 & 415 & 702 & 662 & 1057 \\ \midrule
\multicolumn{1}{r|}{ESP32, TTGO} & 1x 240 MHz & 520 KB & WiFi, \faBluetooth~4.2 & 366 & 427 &  &  \\
\multicolumn{1}{r|}{ESP8266, Feather Huzzah} & 1x 80 MHz & 80 KB & WiFi & 426 & 1321 &  &  \\
\multicolumn{1}{r|}{Feather M0} & 1x 48 MHz & 32 KB & Optionally WiFi, LoRa & 25 & 29 &  &  \\
\multicolumn{1}{r|}{Feather 32u4} & 1x 8 MHz & 2 KB & Optionally LoRa & 24 & 27 &  &  \\
\multicolumn{1}{r|}{Waspmote} & 1x 14.74 MHz & 8 KB &  & 145 & 150 &  &  \\\bottomrule
\end{tabular}
\end{table*}


==> eval_tabs/radio_power.tex <==
\begin{table}[]
\centering
\caption{Power consumption of MCUs including radio transceivers}
\label{sec:eval:radio:power}
\begin{tabular}{@{}rrr@{}}
\toprule\multicolumn{1}{r|}{} & \multicolumn{2}{c}{\textbf{Power} in mW}\\ 
\multicolumn{1}{r|}{} & Mean & Max\\ 
\midrule 
\multicolumn{1}{r|}{ESP32, TTGO, WiFi} & 591 & 1353 \\
\multicolumn{1}{r|}{ESP8266, Feather Huzzah, WiFi} & 405 & 2118 \\
\multicolumn{1}{r|}{Feather M0, WiFi} & 475 & 1577 \\
\multicolumn{1}{r|}{ESP32, TTGO, LoRa} & 235 & 816 \\
\multicolumn{1}{r|}{Feather M0, LoRa} & 45 & 528 \\
\multicolumn{1}{r|}{Feather 32u4, LoRa} & 47 & 568 \\\bottomrule
\end{tabular}
\end{table}


==> eval_tabs/sensors.tex <==
\begin{table}[H]
\centering
\caption{Overview of different Sensors}
\label{sec:eval:sensors:power}
\begin{tabular}{@{}rlrr@{}}
\toprule\multicolumn{1}{r|}{} & \textbf{Function} & \multicolumn{2}{c}{\textbf{Power} in mW}\\ 
\multicolumn{1}{r|}{} &  & Mean & Max\\ 
\midrule 
\multicolumn{1}{r|}{MAX30105} & Particle & 19 & 145 \\
\multicolumn{1}{r|}{CCS811} & VOC, TVOC, eCO2 & 52 & 186 \\
\multicolumn{1}{r|}{PIR} & PIR & 51 & 55 \\
\multicolumn{1}{r|}{SIM28 GPS} & GPS & 250 & 302 \\
\multicolumn{1}{r|}{BME280} & \begin{tabular}[c]{@{}l@{}}Temp., Baro., Humidity\end{tabular} & 56 & 65 \\
\multicolumn{1}{r|}{MICS-2714} & NO2 & 42 & 45 \\
\multicolumn{1}{r|}{MICS-5524} & CO & 41 & 60 \\
\multicolumn{1}{r|}{AMG8833} & IR thermal & 179 & 2248 \\
\multicolumn{1}{r|}{Envirophat} & \begin{tabular}[c]{@{}l@{}}Temp., Baro., Color, \\ Accel., Magnetometer\end{tabular} & 180 & 1868 \\
\multicolumn{1}{r|}{Pi Camera NV} & Night Vision Camera & 1173 & 2290 \\
\multicolumn{1}{r|}{Pi Camera v2.1} & Camera & 393 & 2231 \\\bottomrule
\end{tabular}
\end{table}

